The Proper Motion of Strongly Lensed Binary Neutron Star Mergers in LIGO/Virgo/Kagra can be Constrained by Measuring Doppler Induced Gravitational Wave Dephasing

Strongly lensed binary neutron star (NS-NS) mergers are expected to be observed once LIGO/Virgo/Kagra reaches the planned A+ or proposed A\# sensitivity. We demonstrate that the relative transverse velocity of the source-lens system can be constrained by comparing the phase of the two associated gravitational wave (GW) images, using both semi-analytical and numerical Bayesian methods. For A+ sensitivity, a one-sigma NS-NS merger signal in magnification $(\mu=200)$ and redshift $(z_{\rm S}=1)$ will carry a marginally detectable dephasing signature for a source transverse velocity of $\sim 1800$ km/s. This is comparable to the velocity dispersion of large galaxy clusters. Assuming the same population distribution, the most likely source parameters of $\mu=100$ and $z_{\rm S}=1.4$ are always expected to showcase detectable dephasing imprints for A\# sensitivity, provided they are moving with transverse velocities larger than $\sim 2000$ km/s. We conclude that a first measurement of the relative transverse velocity of a source via GW dephasing methods is likely only a few years away.

==> Reply.tex <==
We thank the referee for the positive an concise review of our work. We have addressed the points and hope that the manuscript warrants publication in Apj.

We have addressed the minor points by:
1) Moving the definition of Q.
2) Adding references to the A+ and A# curves
3) Removing the solar mass unit from Fig. 2
4) Adding some clarifying sentences.

Many thanks for spotting these!

Regarding the referee's major point:
We agree with the referee that we did not spell out what entirely novel measurements are made possible by the methodology we propose.

As the referee recognised, our aim was to provide a solid but concise case for the feasibility of the proposed measurements. The most immediate novel aspect is the possibility of a "dark" measurement of galaxy peculiar velocities/velocity distribution, based on GW only. Whether this is truly novel or only complementary to light based observations is not immediately obvious to us (An analogy would be GW based measurements of the Hubble constant). Another important aspect however, is that not including such dephasing prescriptions could lead to a misidentification of the GW signal.

While we do have ideas about truly novel measurements, especially in combination with multimessenger observations, we did not comment on them here as they are simply speculations. To address the reviewers concerns, we attempted to make our conclusions more precise in the new or rephrased red sections.


Nevertheless, it is arguably interesting in itself to be able to use GW measurements to constrain environmental properties of the merging sources. We opted for leaving this flavouring in the text, as it reflects our personal view and does not affect the actual results, while also attempting to address the reviewers concerns. If the reviewer believes that a more substantial rewriting is needed, we would be open to do so in a further round of reviews.


